Vickrey Auctions for Irregular Distributions

The classic result of Bulow and Klemperer \cite{BK96} says that in a single-item auction recruiting one more bidder and running the Vickrey auction achieves a higher revenue than the optimal auction's revenue on the original set of bidders, when values are drawn i.i.d. from a regular distribution. We give a version of Bulow and Klemperer's result in settings where bidders' values are drawn from non-i.i.d. irregular distributions. We do this by modeling irregular distributions as some convex combination of regular distributions. The regular distributions that constitute the irregular distribution correspond to different population groups in the bidder population. Drawing a bidder from this collection of population groups is equivalent to drawing from some convex combination of these regular distributions. We show that recruiting one extra bidder from each underlying population group and running the Vickrey auction gives at least half of the optimal auction's revenue on the original set of bidders.

==> lower_bound.tex <==


\section{Lower Bound}\label{app:lowerBound}
The optimality (or 1-approximation) 
obtained by Bulow-Klemperer~\cite{BK96} cannot be achieved with our
bidder augmentation procedure for our general non-i.i.d irregular setting. The lower bound of $4/3$ given by 
Hartline and Roughgarden~\cite{HR09} for non-i.i.d regular settings directly translates to a lower bound in our more general setting too.  
An interesting question is whether optimality can be achieved for the i.i.d. irregular case. We show that a Vickrey auction 
with the extra bidders gives less revenue than the optimal auction that is allowed to discriminate bidders by identifying prior to the auction from which regular distribution they are coming from. Specifically, we give an instance where the optimal auction with
discrimination for an irregular distribution that is a mixture of two regular distributions is strictly higher than the Vickrey auction with two extra 
bidders each coming from one of the regular distributions. An interesting question is whether optimality can actually
be achieved with respect to the optimal mechanism that is not allowed to discriminate. That is the optimal auction is Myerson's auction~\cite{M81} for the i.i.d irregular instance. We leave it as an interesting open question.

Our lower bound is based on the lower bound for sub-optimality of duplicating agents presented
in Hartline and Roughgarden~\cite{HR09}. Specifically it was shown that in an auction with two bidders where
bidder $1$ has deterministically value $1$ and bidder two is distributed according to an almost
equal revenue distribution $F_2(x)=1-\frac{1}{x+1}$, then the Vickrey auction after duplicating 
the bidders is only a $4/3$ approximation to the optimal revenue before duplication. 

Using the above example we construct the following instance: Consider an i.i.d. instance among
$2$ bidders where each bidder's value is $1$ with probability $1/2$ and is distributed according
to $F_2(x) = 1-\frac{1}{x+1}$ with probability $1/2$. Such a distribution is irregular and is a convex combination of the two regular ones. 
The revenue curve of the above irregular distribution is the following:
\begin{figure}[h]
\centering
\includegraphics[scale=.6]{lower_bound_revenue_curve.eps}
\end{figure}

Suppose we insert two extra bidders where one bidder has value $1$ and the other is distributed according
to $F_2$ and then run the Vickrey auction. 

First we get that the expected optimal revenue if the auctioneer could discriminate prior to the auction
is at least as much as the following: if he finds that both players come from the equal revenue 
then the optimal revenue is at least $2$. This is because the auctioneer could run a posted price mechanism
with a huge posted price of $H$. The revenue he will get is $H(1-(1-\frac{1}{H+1})^2)=H(1-\frac{H^2}{(H+1)^2})=H\frac{2H+1}{(H+1)^2}$.
As $H$ goes to infinity the above revenue approaches $2$. Hence, the optimal revenue is at least $2$.

If he finds that both come from the deterministic distribution then the revenue is $1$. If 
the seller finds out that one player comes from $F_2$ and the other is deterministic, then he
can make a profit of $\approx 2$ : 
he makes an offer of $H$ to the $F_2$ bidder and if that bidder rejects he makes an offer of 
$1$ to the low bidder. Hence, the expected revenue if the bidder could discriminate prior to 
the auction is: $\frac{1}{4}+\frac{1}{4}2+\frac{1}{2}2=1.75$. 

Now we analyze the revenue of the Vickrey auction with two extra bidders (one with value $1$ 
and the other drawn from $F_2$). When both initial bidders have value $1$ the revenue of
the auction is $1$, since the second highest value is deterministically $1$. When both
initial bidders have value drawn from $F_2$, then the auction has revenue of $z> 1$ if the second
of the three equal revenue bidders has value above $z$, it has revenue $1$ if only one
of the equal revenue bidders is above $1$ and it has revenue $z<1$ if the maximum of the equal revenue
bidders has value $z$. Hence, the revenue has distribution:
\begin{align*}
F_r(z)=\begin{cases}
1-3(1-F_2(z))^2F_2(z)-(1-F_2(z))^3=\frac{z^3+3z^2}{(z+1)^3} & \text{if } z\geq 1\\
F_2(z)^3 = \frac{z^3}{(z+1)^3} & \text{if } z<1
\end{cases}
\end{align*}

Hence, the expected revenue will be: 
\begin{align*}
\int_0^1 1-\frac{z^3}{(z+1)^3} dz + \int_1^\infty \frac{3z+1}{(z+1)^3} dz=\frac{1}{8}+\ln(8)\approx 2.2
\end{align*}

Last, it yields a revenue of only $\frac{3}{2}$ when the bidders come from different distributions (see~\cite{HR09}). Hence, the expected revenue of the Vickrey auction with the two extra bidders is approximately $\frac{1}{4}+\frac{1}{4}2.2+\frac{1}{2}\frac{3}{2}=1.55.$

%Now we move on to examine the optimal revenue of this irregular iid setting. 

%Hence, we observe that to iron the revenue curve we have to treat all the people below maximum of 
%the revenue curve alike and all the people above too, until some very high point (zoomed in region) 
%after which the revenue function is already concave and we don't iron. In addition, anyone below the reserve is 
%never allocated. 
%
%Hence, the optimal auction looks as follows: When two people are above $H$ award it to the highest at the price of the second highest. When one person is above $H$ then award it to him: if no one is in the region 
%$[1,H]$ the award it at a price of $1$ else at a price of $(H+1)/2$. When no one is above
%$H$ then if one or more people are in the region $[1,H]$ award it to one of them randomly at the price of $1$.
%
%The expected revenue from player $2$ of the above auction is as follows: 
%\begin{align*}
%R_2=~&Pr[v_1<1]Pr[v_2\geq 1] + Pr[v_1\in [1,H]](\frac{1}{2}Pr[v_2\in [1,H]]+\frac{H+1}{2}Pr[v_2>H])+
%Pr[v_1>H]E[R_2|v_1>H]\\
%=~& \frac{1}{8}\frac{7}{8}+\frac{1}{2}Pr[v_1\in [1,H]](Pr[v_2\geq 1]+H Pr[v_2>H])+
%\int_H^\infty \int_{v_1}^\infty v_1 dF(v_2) dF(v_1)\\
%=~& \frac{1}{8}\frac{7}{8}+\frac{1}{2}\frac{1}{4}(1+F_2(H))\left(\frac{7}{8}+H\frac{1}{4}(1-F_2(H))\right)
%+\int_H^\infty v_1 Pr[v_2>v_1] dF(v_1)\\
%=~&  \frac{1}{8}\frac{7}{8}+\frac{1}{2}\frac{1}{4}\frac{2H+1}{H+1}\left(\frac{7}{8}+\frac{1}{4}\frac{H}{H+1}\right)
%+\int_H^\infty v_1 \frac{1}{4}\frac{1}{v_1+1}\frac{1}{4}\frac{1}{(v_1+1)^2} dv_1\\
%=~& \frac{1}{8}\frac{7}{8}+\frac{1}{2}\frac{1}{4}\frac{2H+1}{H+1}\left(\frac{7}{8}+\frac{1}{4}\frac{H}{H+1}\right)
%+\frac{1}{4}\frac{1}{4}\frac{1}{2}\frac{2H+1}{(H+1)^2}
%\end{align*}
%
%Observe that since all people above the reserve are treated equally, this corresponds
%to just a posted price mechanism: I pick an order of the people and offer them a reserve price. Thus
%we just need to optimize over the offer price $H$. The expected revenue from any offer price $H>1$  
%is $H (1-(\frac{3}{4}+\frac{1}{4}F_2(H))^2)$. The limit of the above process as $H$ goes to infinity 
%is $1$. Hence, in this irregular case the optimal revenue is $1$. Thus the English auction with the 
%extra bidders outperforms the optimal auction. 
%
%We need to find an example where the above doesn't happen!!


==> regular.tex <==
%\section{Extension Theorem for Non-iid Regular Settings}
Before proving our main result for 
non-i.i.d irregular settings in Section~\ref{sec:irregular}, in this section we
first prove a version of Bulow-Klemperer's result for non-i.i.d regular settings.
Hartline and Roughgarden~\cite{HR09} show that in a non-i.i.d regular setting,
recruiting $n$ additional bidders one from each distribution and running Vickrey
on the $2n$ bidders gives at least half of the optimal revenue obtainable from
the original $n$ bidders. In this section we show that when the number of
distinct (regular) distributions among the original $n$ bidders is $k$, then
revenue of the standard Vickrey auction among $n+k$ bidders, where the extra $k$
bidders are drawn one each from the $k$ distinct regular distributions among the
original $n$ bidders, obtains at least half of the revenue obtained by the
optimal auction among the original $n$ bidders. We show this by showing that the two auctions are 
commensurate in the sense introduced by Hartline and Roughgarden~\cite{HR09}.

\begin{defn}
An auction $M'$ is commensurate to $M$ if:
\begin{align}
\E[\phi_{W'}(v_{W'})|W'\neq W]\geq~& 0 \label{eq:com_1}\\
\E[\phi_{W}(v_{W})|W'\neq W]\leq~& \E_{\vals',\vals}[p_{W'}|W'\neq W] \label{eq:com_2}
\end{align} 
where $W',W$ are the winners of $M',M$ respectively and $p_{W'}$ is the
price paid by the winner of $M'$. 
\end{defn}

\begin{theorem}[Hartline and Roughgarden~\cite{HR09}]\label{thm:commensurate} If mechanism $M'$ is commensurate
to $M$ then $R^M \leq 2R_{M'}$
%\begin{align*}
%R_{M'}\geq \frac{1}{2}R_{M}
%\end{align*}
where $R_{M'}, R_M$ are the expected revenues of mechanisms $M'$ and $M$. (see proof in appendix)
\end{theorem}

We now show that the optimal auction among $n$ bidders is commensurate to
Vickrey auction among $n+k$ bidders.

\begin{lemma}\label{lem:commensurateExtension}
Let $\{F_1,\ldots,F_k\}$ be a set of regular distributions. Consider a setting 
with $n$ bidders where each bidder's valuation is distributed independently and
according to any one of the distributions $F_i$. Let $M$ be the optimal auction among
$n$ bidders and $SP_{n+k}$ be the second price auction with $k$ additional bidders
where each additional bidder comes from a different distribution among the $F_i$'s. Then
$R_{M}\leq 2R_{SP_{n+k}}$
\end{lemma}
\begin{proof}
We show that $M$ is commensurate to $SP_{n+k}$. Let $\vals$ 
denote the valuation profile of the initial $n$ players and $\vals'$ the valuation profile of the 
extra $k$ players. Let $R(\vals,\vals')$ and $S(\vals,\vals')$ denote the winners of auction $M$ and $SP_{n+k}$ respectively. 
Note that $R(\vals,\vals')$ is independent of $\vals'$. We show that: 
\begin{align}
\E_{\vals,\vals'}[\phi_{S(\vals,\vals')}(v_{S(\vals,\vals')})|S(\vals,\vals')\neq
R(\vals,\vals')]\geq~&
0\label{eqn:virtual}\\
\E_{\vals,\vals'}[\phi_{R(\vals,\vals')}(v_{R(\vals,\vals')})|S(\vals,\vals')\neq R(\vals,\vals')]\leq~&
\E_{\vals,\vals'}[p_{S(\vals,\vals')}|S(\vals,\vals')\neq R(\vals,\vals')]\label{eqn:price}
\end{align}
where $p_S$ is the price paid by the winner of the second price auction. 

We first prove the relatively easy inequality~\eqref{eqn:price}. By definition of virtual
values, we know that for any distribution $F$ and any $v$: $\phi(v) \leq v$.
Conditioned on the fact that the winner of the optimal auction $M$ is not the winner of the second price
auction, we have that the price paid in the second price auction is at least the
value of the winner of optimal auction, which is at least the virtual value of
the same. Hence inequality~\eqref{eqn:price} holds point-wise. 

We now prove inequality~\eqref{eqn:virtual}. Conditioned on any value profile $\vals$
of the initial $n$ bidders we show that in expectation over the value profile of
the extra $k$ bidders the inequality holds, i.e.,
\begin{align*}
\E_{\vals'}[\phi_{S(\vals,\vals')}(v_{S(\vals,\vals')})|S(\vals,\vals')\neq R(\vals,\vals'),\vals]\geq~& 0
\end{align*}

Let $N_t$ denote the set of bidders among the $n+k$ bidders that have
distribution $F_t$. For each $t$ we show that when $S(\vals,\vals') \in N_t$, the
expected virtual value $\phi_{S(\vals,\vals')}(v_{S(\vals,\vals')})$ is non-negative. 
If $S(\vals,\vals')\in N_t$, the highest value bidder in $N_t$ is winner, and by
regularity of distributions, the highest virtual value bidder in $N_t$ is
the winner. Hence, we have
\begin{align*}
&\E_{\vals'}[\phi_{S(\vals,\vals')}(v_{S(\vals,\vals')})|S(\vals,\vals')\neq R(\vals,\vals'), S(\vals,\vals')\in
N_t,\vals]\\
&\qquad=\E_{\vals'}[\max_{i\in N_t}\phi_t(v_i)|S(\vals,\vals')\neq R(\vals,\vals'), S(\vals,\vals')\in
N_t,\vals],
\end{align*}
where $\phi_t(\cdot)$ denotes the virtual value function associated with the regular distribution $F_t$. 

We now further condition on whether or not $R(\vals,\vals')\in N_t$. If $R(\vals,\vals')\in N_t$
then some player in $N_t$ must have non-negative virtual value, and thus the the maximum of virtual
values in $N_t$ will be non-negative, thus establishing the required inequality. 
We are left with the case where $R(\vals,\vals')\notin N_t$. Once we condition on $R(\vals,\vals')\notin N_t$ and 
$S(\vals,\vals')\in N_t$, the event $S(\vals,\vals')\neq R(\vals,\vals')$ is redundant. Hence,
we need to show that
\begin{align*}
\E_{\vals'}[\max_{i\in N_t}\phi_t(v_i)|R(\vals,\vals')\notin N_t, S(\vals,\vals')\in N_t,\vals] \geq 0
\end{align*}

Let $e_t$ be the extra bidder drawn from $F_t$ and let $v_t'$ be the value of 
$e_t$. Let $\vals_{-t}'$ denote the valuation profile of the remaining extra bidders. 
Since the winner of the optimal auction on $n$ bidders doesn't depend on the values of the new
bidders, the event $R(\vals,\vals')\notin N_t$ doesn't affect the distribution of $v_t'$.  
Conditioned on $\vals_{-t}'$ and $\vals$, $S(\vals,\vals')\in N_t$ if and only if $v_t'$ is such
that the highest bidder from $N_t$ is the highest bidder overall. I.e., there
is some threshold $\theta(\vals,\vals_{-t}')$ such that if and only if $v_t' \geq
\theta(\vals,\vals_{-t}')$ we have $S(\vals,\vals') \in N_t$. This threshold is zero if $\max_{j
\in N_t\setminus\{e_t\}}v_j = \max_{j \in [n+k]\setminus\{e_t\}}v_j$, and otherwise it is equal to
$\max_{j\in[n+k]\setminus\{N_t\setminus\{e_t\}\}} v_j$. By regularity of $F_t$,
such a threshold on value, translates to a threshold on virtual values, i.e. 
$\phi_t(v_t')$ is greater than or equal some threshold $\phi_t(\theta)$. In sum
we have
\begin{align}
\E_{v_t'}[\max_{i\in N_t}\phi_t(v_i)|R(\vals,\vals')\notin N_t, S(\vals,\vals')\in N_t,\vals_{-t}',\vals]
=~& \E_{v_t'}[\phi_t(v_t')|S(\vals,\vals')\in N_t,\vals_{-t}',\vals]\nonumber\\
=~& \E_{v_t'}[\phi_t(v_t')|\phi_t(v_t')\geq
\phi_t(\theta)]\label{eqn:commensurateFinal}
\end{align}

We know that the expected virtual value of any distribution is the lower bound
of the support of the distribution, which is non-negative since valuations are
non-negative. Hence the expected virtual value conditioned on a lower bound on virtual value
is also non-negative. Hence, the expression in the RHS of
equation~\eqref{eqn:commensurateFinal} is non-negative. This gives us:
\begin{align*}
\E_{v_t'}[\phi_{S(\vals,\vals'}(v_{S(\vals,\vals')})|S(\vals,\vals')\neq R(\vals,\vals'), S(\vals,\vals')\in N_t,\vals_{-t}']\geq 0
\end{align*}
Taking expectation over all $\vals_{-t}'$ we get:
%\begin{align*}
$\E_{v'}[\phi_{S(\vals,\vals'}(v_{S(\vals,\vals')})|S(\vals,\vals')\neq R(\vals,\vals'), S(\vals,\vals')\in N_t]\geq 0.$
%\end{align*}
Since the events $\mathcal{E}_t=\{S(\vals,\vals')\in N_t\}$ are disjoint for each $t$ and 
their union is the whole probability space, equation~\eqref{eqn:virtual} stands
proved.
\end{proof}

\paragraph{\textbf{Vickrey auction with single reserve for Non-i.i.d Regular settings.}}
Hartline and Roughgarden~\cite{HR09} show that the Vickrey auction with an 
anonymous reserve price gets a $4$-approximation to the optimal revenue in any
non-i.i.d regular environment. 
One of the implications of Lemma~\ref{lem:commensurateExtension} is that it
shows how the performance of Vickrey with a single reserve
price improves if the non-i.i.d environment has at most $k$ distinct distributions. 
Specifically suppose that the population of $n$ bidders are divided into $k$
groups of size $n_1,n_2\dots n_k$, with $n_i\geq t$ for all $i$. In such a
setting, if instead of adding $k$ extra bidders, suppose we place a reserve
which follows the distribution of $\max_{i\in[k]}v_i$. Call this auction
$SP_n(R)$. Whenever the winner of the auction $SP_{n+k}$ is among the original
$n$ bidders, the expected revenue of $SP_{n+k}$ and $SP_n(R)$ are the same.
Also, the probability that the winner comes from the original $n$ bidders is at
least $\frac{t}{t + 1}$. Thus
$SP_n(R)$ gets at least a $\frac{1}{2}\frac{t}{t + 1}$ fraction of the revenue of $SP_{n+k}$.
Specifically when all the $n_i$'s are equal, we have this fraction to be
$\frac{1}{2}\frac{n}{n+k}$. At $k = n$, we get the Hartline and Roughgarden~\cite{HR09} bound of $4$ and at $k=1$, the bound is almost $2$.  

\begin{corollary}
In a single-item auction for non-i.i.d regular distributions, when there are $k$ distinct regular distributions with $n_i\geq t$ bidders following distribution $F_i$, Vickrey auction with a single reserve gets at least a $\frac{1}{2}\frac{t}{t+ 1}$ fraction of the optimal revenue from the original bidders.
\end{corollary}



In addition, our result implies an interesting revenue guarantee for the completely prior-independent Vickrey auction with no reserve in non-i.i.d regular settings.
Suppose that $t\geq2$ then we show that a Vickrey auction with no reserve is a $\frac{1}{2}\frac{t-1}{t}$ approximation to optimal revenue.

\begin{corollary}\label{cor:vickrey}
In a single-item auction for non-i.i.d. regular distributions, when there are $k$ distinct distributions with $n_i\geq t$ bidders following $F_i$, the
Vickrey auction gets at least a $\frac{1}{2}\frac{t-1}{t}$ fraction of the optimal revenue. (see proof in appendix)
\end{corollary}


